Budget-Constrained Online Retrieval-Augmented Generation: The Chunk-as-a-Service Model

Large Language Models (LLMs) have revolutionized the field of natural language processing. However, they exhibit some limitations, including a lack of reliability and transparency: they may hallucinate and fail to provide sources that support the generated output. Retrieval-Augmented Generation (RAG) was introduced to address such limitations in LLMs. One popular implementation, RAG-as-a-Service (RaaS), has shortcomings that hinder its adoption and accessibility. For instance, RaaS pricing is based on the number of submitted prompts, without considering whether the prompts are enriched by relevant chunks, i.e., text segments retrieved from a vector database, or the quality of the utilized chunks (i.e., their degree of relevance). This results in an opaque and less cost-effective payment model. We propose Chunk-as-a-Service (CaaS) as a transparent and cost-effective alternative. CaaS includes two variants: Open-Budget CaaS (OB-CaaS) and Limited-Budget CaaS (LB-CaaS), which is enabled by our ``Utility-Cost Online Selection Algorithm (UCOSA)''. UCOSA further extends the cost-effectiveness and the accessibility of the OB-CaaS variant by enriching, in an online manner, a subset of the submitted prompts based on budget constraints and utility-cost tradeoff. Our experiments demonstrate the efficacy of the proposed UCOSA compared to both offline and relevance-greedy selection baselines. In terms of the performance metric-the number of enriched prompts (NEP) multiplied by the Average Relevance (AR)-UCOSA outperforms random selection by approximately 52% and achieves around 75% of the performance of offline selection methods. Additionally, in terms of budget utilization, LB-CaaS and OB-CaaS achieve higher performance-to-budget ratios of 140% and 86%, respectively, compared to RaaS, indicating their superior efficiency.

==> Algorithm/Algorithm.tex <==
%\subsection{The Online Algorithm}\label{sec:Algorithm}
\subsection{UCOSA}\label{sec:Algorithm}

Under the online settings, the prompts are fed to the LB\_CaaS RAG as a stream (\emph{i.e.,} one by one). For each prompt, an initial set of chunks are retrieved (by the Retriever stage) based on their Relevance score, $R_{ij}$. At the Chunk Selection stage, a decision must be made to choose, at most, one chunk to enrich the prompt, considering the achieved Relevance score, the price $P_{ij}$, and the available budget $B$. A decision for a prompt must be made before considering the next prompt, and these decisions cannot be revoked afterwards. To meet these requirements, we propose the Utility-Cost Online Selection Algorithm (UCOSA).   

Before we state the details of UCOSA, some assumptions must be stated:
\begin{itemize}
	\item There exists non-trivial bounds on the values of $\frac{R_{ij}}{P_{ij}}$. That is, $0 < L \leq \frac{R_{ij}}{P_{ij}} \leq U < \infty$.
	\item $\frac{P_{ij}}{B} \leq \epsilon$, where $\epsilon$ is close to 0. 
\end{itemize}
The first assumption means that neither the Relevance score can be infinite, nor the price can be 0. Otherwise, the solution becomes trivial (by selecting the chunk with the infinite score, or selecting the chunk with a zero price). The second assumption states that the price of a chunk is relatively small compared to the available budget.

Now we state the details of UCOSA. Let $z_i$ be the fraction of budget used when the $i$-th prompt arrives, and define $\Psi(z_i) = \big({Ue/L}\big)^{z_i} (L/e)$, where, $e$ is the natural number. Let $Q_i$ be the set of chunks that satisfy $\frac{R_{ij}}{P_{ij}} \geq \Psi(z_i)$. If $Q_i$ is empty, the $i$-th prompt is passed to LLM without enrichment. Else, we pick the chunk from $Q_i$ that gives the maximum Relevance score, and enrich the prompt with that chunk. UCOSA is shown in Algorithm~\ref{alg:alg1}.

\begin{algorithm}
	\caption{UCOSA} \label{alg:alg1}
	\begin{algorithmic}[1]
		\STATE{Initially, $z_i = 0$}
		\STATE{When prompt $i$ arrives, calculate $z_i, \Psi(z_i)$}
		\STATE{Fetch the relevant chunks $\mathcal{J}_i$}
		\STATE{Set $Q_i = \{j \in \mathcal{J}_i \vert \frac{R_{ij}}{P_{ij}} \geq \Psi(z_i)\}$}
		\IF{$Q_i$ is empty}
		\STATE{Pass the prompt to LLM without enrichment}
		\ELSE
		\STATE{find $\hat{j} = argmax_{j \in Q_i} R_{ij}$}
		\STATE{enrich prompt $i$ with chunk $\hat{j}$}
		\ENDIF
		
	\end{algorithmic}
\end{algorithm}

==> Algorithm/CaaS.tex <==
\section{Chunk-as-a-Service (CaaS): Proposed RAG Variants}
\label{sec:proposed_RAG_variants}

This section details our proposed work. First, we introduce the Open-Budget CaaS (OB-CaaS) RAG, the basic variant. Then, we present the limited-budget CaaS (LB-CaaS) RAG, the enhanced variant. 


\subsection{Proposed Open-Budget CaaS (OB-CaaS) RAG Variation}
\label{sec:proposed_OB-CaaS}

Chunks are the key building blocks of RAG. Their indexing and retrieval to enrich prompts are the fundamental aspects of RAG. However, RaaS overlooks this underlying architecture, which renders it a less efficient business model. It fails to consider the specialty of individual data sources and their associated rate of usage, as well as the variable cost that should be associated with chunks based on factors determined collectively by the data source owner and cloud service provider. In other words, the RAG's building blocks (chunks) are not sufficiently and fairly involved in the calculation of the potential profitability. 

Consequently, RaaS fails to provide granular profitability to data source owners and cloud providers. For example, data source owners, such as book authors, are unable to align their sales with RAG's operational style. Ideally, they would earn profits based on the rate of usage and predetermined prices of chunks associated with their data source. This is a fair approach and contributes to creating quality data source content. That, in turn, enables them to compete more effectively for profit when their data is utilized by RAG.

Therefore, we propose a new cloud-based ``Chunk as a Service'' (CaaS) business model to address the limitations of RaaS. Our proposed CaaS adapts the data source indexing process to assign prices to the indexed chunks based on predetermined criteria set by the cloud service provider and the data source owner. In addition to enabling granular profitability and contributing to quality data source content, CaaS enhances the ownership and privacy of proprietary data. This is because CaaS allows for offering services at the chunk level, which can be easily quantified and measured, unlike providing services at the whole RAG level.


This proposed RAG business model (CaaS), in its basic variation, is considered an Open-Budget CaaS (OB-CaaS) RAG model. It assumes no restrictions on the expected budget for utilizing CaaS and offers a business model that prioritizes chunk relevance for selection, regardless of the associated price, which is a typical option for open-budget users. 

Fig. \ref{fig:proposed_RAG_basic_variation} illustrates the pipeline of our proposed OB-CaaS RAG. It highlights our contributions in the indexing and retrieval stages. Compared to the standard RAG pipeline, where the cost of usage does not consider the actual utilization of chunks, the pipeline of our proposed OB-CaaS considers the cost of chunk utilization. This is due to the predetermined prices assigned to the chunks of the indexed data sources. The cost is simply the total price of the utilized chunks: the retrieved and utilized chunks. The selected chunks are the core factor for measuring the cost. 


Although OB-CaaS RAG excels the standard RAG (RaaS) in many aspects, it still shares some limitations with it, including restricting the accessibility only to users with an open budget sufficient to cover the total price of the utilized chunks. Additionally, OB-CaaS RAG does not incorporate an intelligent retrieval functionality that prioritizes the selection of the chunks based on both relevance and price, making OB-CaaS less cost-effective. These limitations make OB-CaaS RAG restrictive; it prevents users with a limited budget from utilizing it. Therefore, we propose an enhanced variant beyond the OB-CaaS, as explained below (Section \ref{sec:proposed_LB-CaaS}).



\subsection{Proposed Limited-Budget (LB-CaaS) RAG Variation}
\label{sec:proposed_LB-CaaS}


LB-CaaS RAG addresses the shortcomings of OB-CaaS RAG, specifically the relative cost-ineffectiveness and restricted user accessibility. This variant enhances the pipeline of OB-CaaS RAG pipeline as follows:

\textbf{At ''Retriever'' stage}, for each plain prompt in the stream, instead of the typical process of retrieving indexed chunks based on the relevance score and then selecting the most relevant one, the relevant chunks are only retrieved\footnote{The retrieved chunks can be stored in a cache which, after the selection of a chunk, is emptied for the next prompt.}, while the selection process is delegated to a new contributed stage named ``the Chunk's Selection Process'' to optimize the selection considering the remaining budget, chunk's relevance score and chunk's price.


\textbf{At ``the Chunk's Selection Process'' stage}, a chunk is selected, from those that were retrieved, to enrich the prompt. 
The selection can be done using optimization techniques, ``online'' algorithms, or greedy approach, as shown in Section~\ref{sec:Model}. The selection is based on a criteria that depends on the chunks' relevance score, price, and the budget used so far. Multiple chunks may satisfy the criteria, in which case, the chunk with the most relevant score is selected (highlighted with orange color as illustrated in Fig. \ref{fig:proposed_RAG_enhanced_variation}) and passed to another contributed stage named ``Enriching prompts with the selected chunks''. 


\textbf{Stage ``Enriching prompts with the selected chunks (Prompt Online Selection)''} 
begins by checking the availability of a selected chunk associated with each prompt. If a chunk is selected by the previous stage, the associated plain prompt utilizes the RAG's synthesizer component to compose an enriched prompt and pass it to the LLM to get a factual-based output. However,  if none of the chunks were selected, the corresponding plain prompt is switched to the LLM directly, generating traditional output.




==> Algorithm/Model.tex <==
%\section{System Model and Algorithms}\label{sec:Model}
This section details the mathematical modeling of our proposed online selection algorithm (UCOSA), including the settings, optimization technique, algorithmic representation, and competitive ratio analysis
%In this section, we start by detailing the settings of CaaS, followed by the different approaches for chunks' selection, namely: optimization technique, online algorithm, and greedy approach. 

\subsection{Settings}\label{subsec:Settings}
There are $\mathcal{I} = \{1, 2, \ldots, i, \ldots, I\}$ plain prompts and $\mathcal{J} = \{1, 2, \ldots, j, \ldots, J\}$ chunks. Enriching the $i$-th prompt with the $j$-th chunk achieves a relevance score of $R_{ij}$ with a price of $P_{ij}$\footnote{The price of a chunk may be the same, regardless of the prompts. However, we assume a different price for different prompts as a generalization.}. The users (\emph{i.e.,} the providers of the prompts) have a budget $B$. The objective is to find an assignment of prompts to chunks that maximizes the overall Relevance score, without exceeding the budget. 


\subsection{Optimization Technique} \label{sec:optimization_technique}
The problem of chunk selection is formulated as an optimization problem. Let:

$x_{ij}  =\left\{ \begin{array}{rl}
	1 &\mbox{if the $i$-th prompt is enriched}\\
	&\mbox{with the $j$-th chunk}\\
	0 &\mbox{otherwise.}
\end{array}\right.$

Then the optimization becomes:

\begin{equation}
	\max \sum_i \sum_j x_{ij} R_{ij}
\end{equation}  
Subject to:

\begin{align}
	&\sum_i \sum_j x_{ij} P_{ij} \leq B \label{const1}\\
	& \sum_j x_{ij} \leq 1 \quad \forall i \label{const2}
\end{align}

Where Constraint~\eqref{const1} states the budget limit, and Constraint~\eqref{const2} states that a prompt can be enriched with 1 chunk at most. The optimization technique assumes that all information, regarding prompts and chunks, are known in advance. The formulation above is for LB\_CaaS. Note that setting $B \rightarrow \infty$ converts it to OB\_CaaS.

\subsection{Online Selection Algorithm (UCOSA)}
Under the online settings, the prompts are fed to the LB\_CaaS RAG as a stream (\emph{i.e.,} one by one). For each prompt, an initial set of chunks are retrieved (by the Retrieval stage) based on their Relevance score, $R_{ij}$. At the Chunk Selection stage, a decision must be made to choose, at most, one chunk to enrich the prompt, considering the Relevance score, the price $P_{ij}$, and the available budget $B$. Note that $R_{ij}$ and $P_{ij}$ are only known when the prompt is fed to the RAG system, not before. A decision for a prompt must be made before considering the next prompt, and these decisions cannot be revoked afterward. To meet these requirements, we propose the Utility-Cost Online Selection Algorithm (UCOSA).
\shawqi{With respect to UCOSA, the relevance is required to be represented as a scalar. However, the way this scalar is obtained is completely under the control of the service provider. It could be a simple relevance measure, or could be obtained through a weighted function of several variables (e.g., diversity, novelty).
Relevance is a well-established metric used in the literature to calculate the similarity between two texts and is often used interchangeably with the term similarity  \cite{lin2025scorerag,wang2024rear}.
}

UCOSA is a generic algorithm that can be applied in various scenarios using diverse representations of utility and cost. In this work, the utility is represented by the relevance score $R$ of the retrieved chunk, while the cost is represented by the associated price $P$ of each retrieved chunk.
\textcolor{Green}{UCOSA is a specialized online selection variant suited to the settings of our proposed LB-CaaS RAG, where chunks are defined by relevance and price.}
It requires assigning a price at the time of selection (assigning prompts the chunks), while the assignment of prices to the chunks is part of the indexing stage.

Before we state the details of UCOSA, some assumptions must be stated:
\begin{itemize}
	\item There exists non-trivial bounds on the values of $\frac{R_{ij}}{P_{ij}}$. That is, $0 < L \leq \frac{R_{ij}}{P_{ij}} \leq U < \infty$.
	\item $\frac{P_{ij}}{B} \leq \epsilon$, where $\epsilon$ is close to 0. 
\end{itemize}
The first assumption means that neither the Relevance score can be infinite, nor the price can be 0. Otherwise, the solution becomes trivial (by selecting the chunk with the infinite score, or selecting the chunk with a zero price). The second assumption states that the price of a chunk is relatively small compared to the available budget.
\textcolor{Green}{This assumption aligns well with real-world cloud service scenarios, where a predefined budget typically serves multiple requests (storage, computation, or retrieval). Such a realistic assumption helps define an appropriate business model for both service providers and end users. In addition, users usually tend to get services from providers that offer a small price compared to their budget. This low-pricing model is common and widely adopted by cloud service providers, including AWS Lambda \cite{AWS2025}.}

%UCOSA selects the chunk that has a relevance-to-price ratio that is above a budget-dependent threshold.
UCOSA selects chunks with relevance-to-price ratios above a budget-dependent threshold, forming a set of candidate chunks (CCH). From within a CCH, the chunk with the highest relevance score is then selected.

Mathematically speaking, let $z_i$ be the fraction of budget used when the $i$-th prompt is fed to LB\_CaaS, and define $\Psi(z_i) = \big({Ue/L}\big)^{z_i} (L/e)$, where, $e$ is the natural number. Let $Q_i$ be the set of chunks that satisfy $\frac{R_{ij}}{P_{ij}} \geq \Psi(z_i)$. If $Q_i$ is empty, the $i$-th prompt is passed to LLM without enrichment. Else, we pick the chunk from $Q_i$ that gives the maximum Relevance score, and enrich the prompt with that chunk.
\shawqi{So, the impact of UCOSA on threshold $\Psi(z_i)$ (the budget-dependent threshold) is as follows: the more UCOSA selects chunks and uses a higher fraction of the budget, the threshold becomes higher, and UCOSA becomes stricter in selecting the next chunks.}
UCOSA is shown in Algorithm~\ref{alg:LB_CaaS_Rep_Algorithim}.
\begin{algorithm}
	%\caption{Algorithmic representation of the proposed LB-CaaS RAG} 
        \caption{UCOSA} 
	\label{alg:LB_CaaS_Rep_Algorithim}
	\textbf{Inputs:}
	\begin{itemize}
		\item \textbf{Plain\_Prompts:} Stream of plain prompts
		\item \textbf{B:} Allocated Budget
	\end{itemize}
	
	\textbf{Outputs:}
	\begin{itemize}
		\item \textbf{Selected\_Chunks:} A subset of the retrieved chunks 
		\item \textbf{Enriched\_Prompts:} A subset of Plain\_Prompts enriched with their associated selected chunks. 
	\end{itemize}
	
	\begin{algorithmic}[1]
		\STATE{Initially, $z_i = 0$}
		\FOR{Each prompt $i$ in \textbf{Plain\_Prompts}} 
		\STATE{\textbf{Retrieval Stage:}}
		\STATE{fetch the relevant chunks $\mathcal{J}_i$}
		\STATE{\textbf{Selection Stage:}}
		\STATE{Compute $z_i, \Psi(z_i)$}
		\STATE{Set $Q_i = \{j \in \mathcal{J}_i \vert \frac{R_{ij}}{P_{ij}} \geq \Psi(z_i)\}$}
		\STATE{find $\hat{j} = argmax_{j \in Q_i} R_{ij}$}
		\STATE{\textbf{Enrichment Stage:}}
		\IF{No chunk is selected}
		\STATE{Pass the prompt to LLM without enrichment}
		\ELSE
		\STATE{Enrich prompt $i$ with chunk $\hat{j}$}
		\ENDIF
		\ENDFOR
		
	\end{algorithmic}
\end{algorithm}
%Later, in Section~\ref{sec:Proof}, we show that the performance of UCOSA is competitive with respect to the optimization formulation.
Appendix~\ref{sec:Proof} demonstrates that the performance of UCOSA is competitive with respect to the optimization formulation.

\begin{comment}
    \subsection{Heuristic Approach}
%opening sentence
We present two heuristic approaches, which also serve as baselines for the simulation results:

\begin{enumerate}
	\item Relevance-Greedy: In this approach, the prompts are fed to the LB\_CaaS RAG as a stream (\emph{i.e.,} one by one). For each prompt, the relevant chunks are retrieved. The chunk with the highest relevance score and a price less than the remaining budget is selected and used to enrich the prompt. 
	
	\item Budget-Balance: In this approach, the budget is divided equally among the prompts. Then, for each prompt, the chunks with a price less or equal than the allocated budget are retrieved. Among those, the chunk with the highest relevance score is selected to enrich the prompt.
\end{enumerate}
\end{comment}

==> Algorithm/Proof.tex <==
\section{UCOSA's Competitive Ratio Analysis}\label{sec:Proof}
%\subsection{Competitive Ratio Analysis}\label{sec:Proof}
In this section, we show that UCOSA achieves a competitive ratio of $\ln (U/L) + 2$. Moreover, we show that the best competitive ratio achieved by any online algorithm cannot be lower than $\ln (U/L) + 1$. The competitive ratio is a measure of the worst-case performance of the online algorithm compared to the optimal solution. In our work, let $\mathcal{R}_{UCOSA}$ be the total Relevance score achieved by UCOSA, and let $\mathcal{R}_{OPT}$ be the total Relevance score achieved by the optimal solution (the optimization formulation in Section~\ref{sec:optimization_technique}), then we show that 

\begin{displaymath}
	\frac{\mathcal{R}_{OPT}}{\ln (U/L) + 2} \leq \mathcal{R}_{UCOSA} \leq \mathcal{R}_{OPT}
\end{displaymath}

\textcolor{Green}{
The proof starts by examining the sets of prompts enriched with a selected chunk $j$ by the offline algorithm and UCOSA, denoted by $S_j^*$ and $S_j$, respectively. The set $S_j^*$ is partitioned into subsets. Leveraging the properties of $\Psi(z_i)$ and the selection condition of UCOSA (Line 7 of Algorithm 1), we bound the relevance score achieved by each subset compared to the relevance score achieved by UCOSA. Taking the ratio of $\mathcal{R}_{OPT}/\mathcal{R}_{UCOSA}$ over all chunks yield the competitive ratio result.
}

Before delving into the mathematical proof, we note the following properties of the function $\Psi(z_i)$ used in UCOSA:
\begin{itemize}
	\item When $z_i \in [0, \frac{1}{1 + \ln (U/L)}]$, the value of $\Psi(z_i) \leq L$. Therefore, all prompts will be enriched with a chunk.
	\item When $z_i = 1$, the value of $\Psi (z_i) = U$. From the algorithm, no additional prompts will be enriched, and the budget is not violated.
	\item $\Psi(z_i)$ is a monotonically increasing function of $z_i$.
\end{itemize}

We now prove the competitive ratio of UCOSA.
\subsubsection{Proof of Competitive Ratio}
The proof is as follows.
\begin{proof}
	Fix an input sequence $\zeta$. Let $OPT(\zeta)$ and $A(\zeta)$ be the total Relevance score obtained by the optimal offline and UCOSA, respectively. Suppose that when the UCOSA terminates, the fraction of budget consumed to use chunk $j$ is $Z_j$, and let $B_j = Z_j B$. Let $S_j^* , S_j$ be the set of prompts enriched with chunk $j$ by the optimal offline and the UCOSA, respectively.
	
	We partition the set $S_j^*$ into 3 subsets:
	\begin{itemize}
		\item The prompts enriched by both offline and UCOSA with chunk $j$. Denote this by $D_j^* = S_j^* \cap S_j$
		\item The prompts enriched by the offline with chunk $j$, but not enriched by UCOSA. Denote this by $X_j^* = S_j^* \backslash S_j$.
		\item The prompts enriched by the offline with chunk $j$, but enriched with different chunk by UCOSA. Denote this by $Y_j^*$.
	\end{itemize}
	
	For the prompts in $D_j^*$, since it was enriched by UCOSA, then $R_{ij} \geq P_{ij}\Psi(z_i), \forall i \in D_j^*$. The total Relevance score $v(D_j^*)$ of these prompts is:
	\begin{eqnarray}
		v(D_j^*) &= \sum_{i \in D_j^*} R_{ij} \nonumber\\
		&\geq \sum_{i \in D_j^*} P_{ij}\Psi(z_i) \label{eq:eq1}
	\end{eqnarray}
	Since $\Psi(z_i)$ is monotonically increasing, The right hand side of Equation~\eqref{eq:eq1}: 
	\begin{equation}
		\sum_{i \in D_j^*} P_{ij}\Psi(z_i) \leq \sum_{i \in D_j^*} P_{ij}\Psi(Z_j) \leq B\Psi(Z_j) \label{eq:D}
	\end{equation}
	
	For the prompts in $X_j^*$, since these were not enriched by UCOSA, then $R_{ij} \leq P_{ij}\Psi(z_i), \forall i \in X_j^*$. Therefore:
	\begin{eqnarray}
		\sum_{i \in X_j^*} R_{ij} &\leq \sum_{i \in X_j^*} P_{ij}\Psi(z_i) \nonumber\\
		&\leq \sum_{i \in X_j^*} P_{ij}\Psi(Z_j) \nonumber\\
		&\leq \Psi(Z_j)(B - B_j) \label{eq:X}
	\end{eqnarray}
	
	For the prompts in $Y_j^*$, UCOSA enriched the prompt with a different chunk to achieve a higher score. Therefore:
	\begin{displaymath}
		v_{off}(Y_j^*) \leq v_{UCOSA}(Y_j^*) \leq v(S_j), \forall j
	\end{displaymath} 
	where $v_{off}(Y_j^*)$ and $v_{UCOSA}(Y_j^*)$ are the sum of Relevance scores of the set $Y_j^*$ achieved by the optimal offline and UCOSA, respectively. Therefore:
	\begin{equation}
		\sum_j v_{off}(Y_j^*) \leq \sum_j v(S_j) = A(\zeta) \label{eq:Y}
	\end{equation}
	
	There are also the prompts enriched by UCOSA with chunk $j$, but not enriched by the offline algorithm (\emph{i.e.,} the set $S_j \backslash S_j^*$). For these prompts, we have:
	\begin{equation}
		v(S_j \backslash S_j^*) = \sum_{i \in S_j \backslash S_j^*} R_{ij} \geq \sum_{i \in S_j \backslash S_j^*}P_{ij}\Psi(z_i) \label{eq:G}
	\end{equation}
	
	Note that $OPT(\zeta) = \sum_j \big(v(D_j^*) + v(X_j^*) + v_{off}(Y_j^*)\big)$, and $A(\zeta) = \sum_j \big(v(D_j^*) + v(S_j \backslash S_j^*)\big)$. The competitive ratio is:
	\begin{eqnarray}
		\frac{OPT(\zeta)}{A(\zeta)} &= \frac{\sum_j \big(v(D_j^*) + v(X_j^*) + v_{off}(Y_j^*)\big)}{\sum_j \big(v(D_j^*) + v(S_j \backslash S_j^*)\big)} \nonumber \\
		&\leq \frac{\sum_j \big(v(D_j^*) + v(X_j^*)\big)}{A(\zeta)} + \frac{A(\zeta)}{A(\zeta)} \nonumber \\
		&\leq \frac{\sum_j \big[\sum_{i \in D_j^*} \big(P_{ij}\Psi(Z_j)\big) + \Psi(Z_j)(B - B_j) \big]}{\sum_j \big[\sum_{i \in D_j^*} \big(P_{ij}\Psi(Z_j)\big) + v(S_j \backslash S_j^*) \big]} + 1 \nonumber\\
		&\leq \frac{\sum_j \big[\Psi(Z_j)B_j + \Psi(Z_j)(B - B_j) \big]}{\sum_j \big[\sum_{i \in D_j^*} \big(P_{ij}\Psi(Z_j)\big) + v(S_j \backslash S_j^*) \big]} + 1 \nonumber \\
		&\leq \frac{\sum_j \Psi(Z_j)B}{\sum_j \big( \sum_{i \in S_j} \Psi(z_i)P_{ij} \big)} + 1\nonumber \\
		&\leq \frac{\sum_j \Psi(Z_j)}{\sum_j \big( \sum_{i \in S_j} \Psi(z_i)\Delta z_i \big)} + 1 \label{eq:1}
	\end{eqnarray}
	Where the first inequality is obtained by substituting Equation~\eqref{eq:Y}. The second inequality is obtained by substituting Equation~\eqref{eq:X}, the third inequality is obtained by substituting Equation~\eqref{eq:D}, and the last inequality is obtained by substituting $\Delta z_i = P_{ij}/B$.
	
	For the denominator of Equation~\eqref{eq:1}, we approximate the summation via an integration (since we already assumed that $P_{ij}/B \leq \epsilon$, where $\epsilon \rightarrow 0$). Therefore, for every chunk $j$ we have:
	\begin{eqnarray}
		\sum_{i \in S_j} \Psi(z_i)\Delta z_i &\approx \int_{0}^{Z_j} \Psi(z_i)dz_i \nonumber\\
		&= \int_{0}^{g} Ldz_i + \int_{g}^{Z_j} \Psi(z_i)dz_i \nonumber \\
		&= gL + \frac{L}{e}\frac{(Ue/L)^{Z_j} - (Ue/L)^{g}}{\ln (Ue/L)} \nonumber\\
		&= \frac{L}{e} \frac{(Ue/L)^{Z_j}}{\ln (Ue/L)} \nonumber \\
		&= \frac{\Psi(Z_j)}{\ln (U/L) + 1} \label{eq:2}	  
	\end{eqnarray}
	Where $g = \frac{1}{1 + \ln (U/L)}$.
	
	Substituting Equation~\eqref{eq:2} in Equation~\eqref{eq:1}, we have:
	$\frac{OPT(\zeta)}{A(\zeta)} \leq \frac{\sum_j \Psi(Z_j)}{\frac{\Psi(Z_j)}{\ln (U/L) + 1}} + 1 \leq \ln (U/L) + 2$.
	
	
	Since each of the ratios $\frac{\Psi(Z_j)}{\sum_{i \in S_j} \Psi(z_i)\Delta z_i}$ is less than $\frac{1}{\ln (U/L) +1}$, the last inequality follows.
	
\end{proof}

\subsubsection{Lower Bound Proof}
To prove the lower bound on the competitive ratio, we provide an instance of the problem on which no online algorithm can achieve a better competitive ratio than $\ln(U/L) + 1$.

UCOSA presented above is a deterministic algorithm (\emph{i.e.,} given the same input sequence, UCOSA will produce the exact same output). To prove the competitive ratio, we use Yao's principle. Yao's principle states that deterministic algorithms performs worse than randomized algorithms against an oblivious adversary (one who does not know the outcomes of the random process in the randomized algorithm). Therefore, a lower bound on the randomized algorithm is also a lower bound on the deterministic algorithm.

For any input distribution $\mathcal{F}$ and $\gamma$-competitive randomized algorithm $\mathcal{A}$, we will show that:
\begin{displaymath}
	\frac{1}{\gamma} \leq \min_{\sigma} \frac{\mathbb{E}[\mathcal{A}(\sigma)]}{OPT(\sigma)} \leq \max_{deterministic A} \mathbb{E}_{\sigma \leftarrow \mathcal{F}} \big[ \frac{A(\sigma)}{OPT(\sigma)} \big]
\end{displaymath}

To prove the lower bound, we specify a distribution $\mathcal{F}$ such that:
\begin{equation}
	\max_{deterministic A} \mathbb{E}_{\sigma \leftarrow \mathcal{F}} \big[ \frac{A(\sigma)}{OPT(\sigma)}\big] \leq \frac{1}{\ln(U/L) +1}
\end{equation}

The instance of the problem is defined as follows:
\begin{itemize}
	\item The instance has one chunk.
	\item Fix a parameter $\eta > 0$. Let $k$ be the largest integer such that $(1 + \eta)^k \leq U/L$. Therefore, $k = \lfloor \frac{\ln(U/L)}{\ln(1+\eta)} \rfloor$.
	\item The support of the input distribution $\mathcal{F}$ consist of the instances $I_0, I_1, \ldots, I_k$, where $I_0$ consists of $B$ identical prompts each with price 1 and Relevance score of $L$, and $I_{m+1}$ consists of $I_m$ followed by additional $B$ prompts each with price 1 and a Relevance score $(1+\eta)^{m+1}L$. This means that $I_m \subset I_{m+1}$.
	\item The probabilities of the instances $I_0, I_1, \ldots, I_k$ are defined as follows: $p_k = \frac{1+\eta}{(k+1)\eta + 1}$, and $p_m = \frac{\eta}{(k+1)\eta + 1}, \forall m \in \{0, 1, \ldots, k-1\}$. Note that $\sum_{m=0}^{k} p_m = 1$. 
	\item Define $H = (k+1)\eta + 1$.  
\end{itemize}

\begin{proof}
	Let $b_m$ be the fraction of the budget used for prompts with profits $(1+\eta)^m L$, $m = 0, 1, \ldots, k$. We note that $\sum_{m=0}^{k} b_m \leq 1$ since a proper algorithm will not use more than the available budget. Now, we have:
	
	\begin{eqnarray}
		\mathbb{E}_{\sigma \leftarrow \mathcal{F}} \big[ \frac{A(\sigma)}{OPT(\sigma)} \big]&= \sum_{i=0}^{k} \frac{p_i \sum_{m=0}^{i} (1+\eta)^j b_m}{(1+\eta)^i} \nonumber \\
		&= \sum_{m=0}^{k}b_m \sum_{i=m}^{k} p_i (1+\eta)^{m-i} \nonumber 
	\end{eqnarray}
	
	For any $m$:
	\begin{eqnarray}
		\sum_{i=m}^{k} p_i (1+\eta)^{m-i} &= p_k (1+\eta)^{m-k} + \sum_{i=m}^{k-1} p_i (1+\eta)^{m-1} \nonumber \\
		&= \frac{(1+\eta)^{m-k+1}}{H} + \frac{\eta}{H} \sum_{i=m}^{k-1}(1+\eta)^{m-i} \nonumber \\
		&= \frac{(1+\eta)^{m-k+1}}{H} + \frac{\eta}{H} \frac{(1+\eta) - (1+\eta)^{m-k+1}}{\eta} \nonumber \\
		&= \frac{1+\eta}{H} = \frac{1+\eta}{(k+1)\eta + 1} \nonumber
	\end{eqnarray}
	
	where the second equality comes from substituting the values of $p_m$, and the last equality comes from substituting the value of $H$.
	
	Therefore, we get:
	\begin{eqnarray}
		\mathbb{E}_{\sigma \leftarrow \mathcal{F}} \big[ \frac{A(\sigma)}{OPT(\sigma)} \big] &= \frac{1+\eta}{(k+1)\eta + 1}\sum_{m=0}^{k}b_m \nonumber \\
		&\leq \frac{1+\eta}{(k+1)\eta + 1} \nonumber \\
		&\leq \frac{1+\eta}{\eta \frac{\ln(U/L)}{\ln(1+\eta)} + 1} \nonumber 
	\end{eqnarray}
	where the first inequality comes from $\sum_{m=0}^{k}b_m \leq 1$, and the second inequality comes from substituting the value of $k = \lfloor \frac{\ln(U/L)}{\ln(1+\eta)} \rfloor$.
	
	By taking the limit as $\eta \rightarrow 0$, and noting that $\lim_{\eta \rightarrow 0} \frac{\eta}{\ln(1+\eta)} =1$, we complete the proof.
\end{proof}
